Pointer Life Cycle Types for Lock-Free Data Structures with Memory Reclamation

We consider the verification of lock-free data structures that manually manage their memory with the help of a safe memory reclamation (SMR) algorithm. Our first contribution is a type system that checks whether a program properly manages its memory. If the type check succeeds, it is safe to ignore the SMR algorithm and consider the program under garbage collection. Intuitively, our types track the protection of pointers as guaranteed by the SMR algorithm. There are two design decisions. The type system does not track any shape information, which makes it extremely lightweight. Instead, we rely on invariant annotations that postulate a protection by the SMR. To this end, we introduce angels, ghost variables with an angelic semantics. Moreover, the SMR algorithm is not hard-coded but a parameter of the type system definition. To achieve this, we rely on a recent specification language for SMR algorithms. Our second contribution is to automate the type inference and the invariant check. For the type inference, we show a quadratic-time algorithm. For the invariant check, we give a source-to-source translation that links our programs to off-the-shelf verification tools. It compiles away the angelic semantics. This allows us to infer appropriate annotations automatically in a guess-and-check manner. To demonstrate the effectiveness of our type-based verification approach, we check linearizability for various list and set implementations from the literature with both hazard pointers and epoch-based memory reclamation. For many of the examples, this is the first time they are verified automatically. For the ones where there is a competitor, we obtain a speed-up of up to two orders of magnitude.

==> content/_unused_avoiding_races.tex <==
%!TEX root = ../main.tex

\presection
\section{Atomicity Abstraction}
\label{sec:avoiding-pointer-races}
\label{sec:atomicity-abstraction}
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
Data structure implementations may contain pointer races despite the use of SMR.
The reason is that programmers exploit intricate invariants of the data structure to ensure that pointer-racy actions are guaranteed to be safe. 
Consequently, our type check will fail although the implementation is correct.
To increase the applicability of our type system, % and allow for a successful verification nonetheless, 
we suggest to transform implementations on which the type check fails. 
The goal of the transformation is to avoid the pointer race while retaining all behaviors of the original implementation. 
More precisely, we transform the given program $\aprog$ into another program $\aprogp$ such that $\anobs\allsem[\aprog]\subseteq\anobs\allsem[\aprogp]$.
If $\aprogp$ is free from pointer races, our results apply and we obtain~$\anobs\allsem[\aprogp]\computrel\nosem[\aprogp]$.
Then successful verification for $\nosem[\aprogp]$ carries over to full $\anobs\allsem[\aprog]$. 
%T % because of $\allsem[\aprog]\computrel\nosem[\aprogp]$.

% \begin{figure}
% \begin{tcolorbox}
% 	\begin{subfigure}[b]{.48\textwidth}
% \begin{lstlisting}[style=condensed]
% head = Head;
% if (*) {
% 	protect(head, 0);
% 	assume(head != Head);
% 	// restart procedure
% } else {
% 	atomic {
% 		protect(head, 0);
% 		assume(head == Head);
% 	}
% 	// continue procedure
% }
% \end{lstlisting}
% 		\subcaption{\sw{???}}
% 		\label{fig:atomicity:step-make-atomic}
% 	\end{subfigure}
% 	% \\[4mm]
% 	\hfill
% 	\begin{subfigure}[b]{.48\textwidth}
% \begin{lstlisting}[style=condensed]
% if (*) {
% 	head = Head;
% 	protect(head, 0);
% 	assume(head != Head);
% 	// restart procedure
% } else {
% 	atomic {
% 		head = Head;
% 		protect(head, 0);
% 	}
% 	// continue procedure
% }
% \end{lstlisting}
% 		\subcaption{\sw{???}}
% 		\label{fig:atomicity:step-remove-assumption}
% 	\end{subfigure}
% 	\caption{\sw{???}}
% 	\label{fig:atomicity-msq}
% \end{tcolorbox}
% \end{figure}

% A typical reason for a pointer race is the lack of atomicity.
% For an example, consider \Cref{code:michaelscott_hp:read-head,code:michaelscott_hp:protect-head,code:michaelscott_hp:check-head} of Michael\&Scott's queue from \Cref{fig:michaelscott_hp}.
% There,
% \begin{inparaenum}[(i)]
% 	\item the shared \code{Head} is copied into a local pointer \code{head} (\Cref{code:michaelscott_hp:read-head}),
% 	\item a protection is issued for that local pointer \code{head}  (\Cref{code:michaelscott_hp:protect-head}), and then
% 	\item the procedure is restarted if \code{Head} has changed since it was read out (\Cref{code:michaelscott_hp:check-head}).
% \end{inparaenum}
% This is a common pattern for protecting records using hazard pointers.
% However, the comparison of \code{Head} and \code{head} in \Cref{code:michaelscott_hp:check-head} raises a pointer race: \code{head} may be invalid despite the protection in \Cref{code:michaelscott_hp:protect-head}.
% The reason for this is that \Cref{code:michaelscott_hp:read-head,code:michaelscott_hp:protect-head} are not executed atomically.
% Hence, the record referenced by \code{head} could be retired and freed by another thread before the protection takes place.
% This renders \code{head} invalid and results in the aforementioned pointer race.
% \sw{In fact: \Cref{code:michaelscott_hp:check-head} is an ABA; but I don't think we want to go there.}

\begin{figure}
\begin{tcolorbox}
	\begin{subfigure}[b]{.48\textwidth}
\begin{lstlisting}[style=condensed]
head = Head; $\label[line]{code:racy:read-head}$
protect(head, 0); $\label[line]{code:racy:protect-head}$
if (*) {
	assume(head != Head); $\label[line]{code:racy:check-head-changed}$
	// restart procedure
} else {
	assume(head == Head); $\label[line]{code:racy:check-head-unchanged}$
	// continue procedure
}
\end{lstlisting}~
		\subcaption{Protection pattern from Michael\&Scott's queue. The conditional in \Cref{code:racy:check-head-unchanged} is prone to a pointer race.}
		\label{fig:atomicity:racy}
	\end{subfigure}
	% \\[4mm]
	\hfill
	\begin{subfigure}[b]{.48\textwidth}
\begin{lstlisting}[style=condensed]
if (*) {
	head = Head; protect(head, 0);
	assume(head != Head);
	// restart procedure
} else {
	atomic {
		head = Head; protect(head, 0);
	}
	// continue procedure
}
\end{lstlisting}
		\subcaption{Protection of Michael\&Scott's queue rewritten to avoid pointer races while retaining all behavior.}
		\label{fig:atomicity:atomic}
	\end{subfigure}
	\caption{Making a program more atomic to avoid pointer races while retaining the original behavior.}
	\label{fig:atomicity}
\end{tcolorbox}
\end{figure}

%\Cref{code:michaelscott_hp:read-head,code:michaelscott_hp:protect-head,code:michaelscott_hp:check-head} of Michael\&Scott's queue from \Cref{fig:michaelscott_hp}

To motivate our choice of program transformations, we elaborate on the popular retry idiom, a programming pattern under safe memory reclamation that relies on pointer races.  
Consider \Cref{code:michaelscott_hp:read-head,code:michaelscott_hp:protect-head,code:michaelscott_hp:check-head} of Michael\&Scott's queue from \Cref{fig:michaelscott_hp} the code of which is repeated in \Cref{fig:atomicity:racy} for convenience.
There,
\begin{inparaenum}[(i)]
	\item the shared \code{Head} is copied into a local pointer \code{head} (\Cref{code:racy:read-head}),
	\item a protection is issued for that local pointer \code{head}  (\Cref{code:racy:protect-head}), and then
	\item the procedure is restarted if \code{Head} has changed since it was read out (\Cref{code:racy:check-head-changed}) and continued otherwise (\Cref{code:racy:check-head-unchanged}).
\end{inparaenum}
The comparison of \code{Head} and \code{head} in \Cref{code:racy:check-head-unchanged} raises a pointer race: \code{head} may be invalid despite the protection in \Cref{code:racy:protect-head}.
The reason is that \Cref{code:racy:read-head,code:racy:protect-head} are not executed atomically.
The record referenced by \code{head} could be retired and freed by another thread before the protection takes place. 
This renders \code{head} invalid.  
In fact,  \Cref{code:racy:check-head-unchanged} is an ABA. 
The ABA, however, is harmless in that the reallocated address can safely be accessed. 
(The comparison in \Cref{code:racy:check-head-changed} does not raise a pointer race according to \Cref{def:prf-brief}.)
The retry idiom for protecting records is not limited to hazard pointers but applied in combination with other SMR algorithms as well.

%\sw{In fact: \Cref{code:racy:check-head-unchanged} is an ABA; but I don't think we want to go there.}
To overcome the problem of harmless pointer races, we propose to transform the program into a more atomic version. 
This idea is referred to as \emph{atomicity abstraction} and  well-known in the literature, with contributions ranging from \cite{Lipton75} to~\cite{DBLP:conf/cav/HawblitzelPQT15,DBLP:conf/cav/KraglQ18}.  
We refer the reader to \Cref{sec:related_work} for an overview. 
In the above example, we execute the read and protect atomically, as done in \Cref{fig:atomicity:atomic}. 
While this atomicity cannot be achieved in practice for the performance penalty it brings, it is a useful transformation for verification.
In fact, the transformed code allows for the same (modulo later reclamation) %(or more\footnote{The transformed code can always choose the retry branch. This is not possible in the original code.})
behavior. 
Yet, it is free from pointer races. 
In the following, we develop an atomicity abstraction tailored towards programs with safe memory reclamation. 
We invoke it whenever the type check fails.

The fundamental technique behind atomicity abstraction are movers \cite{Lipton75}.
Intuitively, a command is a mover if it can be reordered with commands of other threads.
This allows for the command to be moved to the next command of the same thread, effectively constructing an atomic block containing the mover and the next command.
There is plenty of work on movers as well that we discuss in \Cref{sec:related_work}.
The difference with existing work is that our programs contain SMR commands the semantics of which depends on the underlying SMR algorithm. 
We propose the following notion of moverness that takes into account an SMR algorithm $\anobs$. 
%To make available movers for our efforts, we show that ordinary mover reasoning carries over to our programming model.
%To make this more precise, we consider two partitions of commands.
%Partition the set of commands into \emph{SMR commands}
%($\enter$, $\exit$, and $\free$) and the remaining \emph{memory commands}. 
Command $\acom$ at location $\aloc$ of program $\aprog$ \emph{right-moves}, if for all computations $\tau.\anact_1.\anact_2$ in $\anobs\allsem[\aprog]$ with $\anact_i=(\athread_i,\acom_i,\anup_i)$ and $\athread_1\neq\athread_2$ and $\acom_1=\acom$ and $\controlof{\athread_1}=\aloc$ we have 
\begin{align*}
\heapcomput{\tau.\anact_1.\anact_2}=\heapcomput{\tau.\anact_2.\anact_1}\quad \text{and}\quad
\freeableof{\tau.\anact_1.\anact_2}{\anadr}\subseteq\freeableof{\tau.\anact_2.\anact_1}{\anadr},\quad \text{for all $\anadr\in\adr$\ .}
\end{align*} 
The equality is the expected requirement that the memories resulting from the two computations coincide.  
The inclusion is SMR specific and requires that when moving $\anact_1$ to the right, we only obtain more behavior, on every address. 

What is remarkable about the definition of moverness is that SMR commands  ($\enter$, $\exit$, $\free$) do not modify the memory (relevant for the equality) while memory commands do not affect the history of the computation (relevant for the inclusion).  
As a consequence, an SMR command $\acom$ always right-moves over a memory command $\acomp$ and vice versa. 
To be precise, this holds as long as $\acomp$ does not change the valuation of pointers used by $\acom$. 
Since only commands $\acomp$ of other threads are considered, this is guaranteed to hold if SMR commands $\acom$ never access shared variables. 
This holds for all SMR algorithms we are aware of. 
One reason is that shared variables are subject to interferences, and hence it is not clear what would be protected.
Another reason is that local variables are cheaper to access. 

It remains to establish moverness for memory commands and for SMR commands.
For a memory command, we remove from the code all SMR commands. 
The result is an ordinary concurrent program (modulo invariants, but they hardly move) to which we apply the moverness proof techniques in the literature~\cite{}. 

For an SMR command to be a mover, we have to establish $\freeableof{\tau.\anact_1.\anact_2}{\anadr}\subseteq\freeableof{\tau.\anact_2.\anact_1}{\anadr}$ for all computations $\tau.\anact_1.\anact_2$ and all addresses $\anadr$. 
Consider the interesting case where both $\anact_1$ and $\anact_2$ execute SMR commands.
Since neither of the actions updates the memory by definition, the histories are of the form $\ahist.\anevent_1.\anevent_2$ resp. $\ahist.\anevent_2.\anevent_1$. 
%Then, $\historyof{\tau.\anact_1.\anact_2}$ is of the form $\historyof{\tau.\anact_1.\anact_2}=\ahist.\anevent_1.\anevent_2$ with $\ahist=\historyof{\tau}$.
%Since neither of the actions updates the memory by definition, we have $\historyof{\tau.\anact_2.\anact_1}=\ahist.\anevent_2.\anevent_1$.
Runs of the SMR automaton $\anobs$ on those histories take the form
\begin{align*}
	(\alocation_0,\varphi)\trans{\ahist}(\alocation_1,\varphi)\trans{\anevent_1}(\alocation_2,\varphi)\trans{\anevent_2}(\alocation_3,\varphi)
	\qquad\text{and}\qquad
	(\alocation_0,\varphi)\trans{\ahist}(\alocation_1,\varphi)\trans{\anevent_2}(\alocation_2',\varphi)\trans{\anevent_1}(\alocation_3',\varphi)
	\ .
\end{align*}
Consequently, it suffices to show that observer state $\alocation_3'$ allows for more behavior than $\alocation_3$.
To prove this, we approximate SMR automata by finite-state automata and check an inclusion.

Our tool integrates several rewriting patterns that introduce atomicity.
They are triggered by pointer races found during the type check and preconditioned by successful moverness checks.
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
% ------------------------------------------------------------------------------------------
\subsubsection*{Loop Peeling}
Related to the above retry idiom are loops that try to publish a newly allocated record. 
Assume the record is referenced by a local pointer $\apvar$. 
Then, $\apvar$ has guarantee $\glocal$ before the publishing loop iteration. 
During the last iteration, when $\apvar$ is published, it loses $\glocal$ because an alias is created. 
To apply Rule~\ref{rule:choice}, however, we need a pre type environment where $\apvar$'s type does not contain~$\glocal$. 
This makes $\glocal$ useless and may require annotations within the loop in case $\apvar$ is accessed. 
Our pragmatic fix for the problem is to peel the last, publishing loop iteration.
That way, the transformed loop maintains $\glocal$ and the peeled iteration removes it. 
The semantics of the program does not change. 
The approach is implemented in our tool.
% \begin{figure}
% \begin{tcolorbox}
% 	\begin{subfigure}[t]{.48\textwidth}
% \begin{lstlisting}[style=condensed]
% head = Head;
% if (*) {
% 	atomic {
% 		@protect(head, 0);@
% 		assume(head != Head);
% 	}
% 	// retry
% } else {
% 	atomic {
% 		@protect(head, 0);@
% 		assume(head == Head);
% 	}
% 	// continue
% }
% \end{lstlisting}
% 		\subcaption{The SMR API call is a right-mover, it can be executed atomically with the subsequent command.}
% 		\label{fig:atomicity-intermediary-steps:protect}
% 	\end{subfigure}
% 	% \\[4mm]
% 	\hfill
% 	\begin{subfigure}[t]{.48\textwidth}
% \begin{lstlisting}[style=condensed]
% @head = *;@
% if (*) {
% 	atomic {
% 		protect(head, 0);
% 		assume(head != Head);
% 	}
% 	// retry
% } else {
% 	atomic {
% 		protect(head, 0);
% 		assume(head == Head);
% 	}
% 	// continue
% }
% \end{lstlisting}
% 		\subcaption{Assignments can be replaced with non-deterministic values without cutting away behavior of the original program.}
% 		\label{fig:atomicity-intermediary-steps:nondet}
% 	\end{subfigure}
% 	\\[2mm]
% 	\begin{subfigure}[t]{.48\textwidth}
% \begin{lstlisting}[style=condensed]
% if (*) {
% 	atomic {
% 		@head = *;@
% 		protect(head, 0);
% 		assume(head != Head);
% 	}
% 	// retry
% } else {
% 	atomic {
% 		@head = *;@
% 		protect(head, 0);
% 		assume(head == Head);
% 	}
% 	// continue
% }
% \end{lstlisting}
% 		\subcaption{Non-deterministic assignments to local variables are right-movers as they are not affected by interfering threads.}
% 		\label{fig:atomicity-intermediary-steps:assign}
% 	\end{subfigure}
% 	% \\[4mm]
% 	\hfill
% 	\begin{subfigure}[t]{.48\textwidth}
% \begin{lstlisting}[style=condensed]
% if (*) {
% 	atomic {
% 		head = *;
% 		protect(head, 0);
% 		assume(head != Head);
% 	}
% 	// retry
% } else {
% 	atomic {
% 		@head = Head;@
% 		protect(head, 0);
% 		assume(head == Head);
% 	}
% 	// continue
% }
% \end{lstlisting}
% 		\subcaption{Non-deterministic assignments followed by assumptions need only assign the assumed value.}
% 		\label{fig:atomicity-intermediary-steps:oldassignagain}
% 	\end{subfigure}
% 	\caption{%
% 		Applying stepwise atomicity abstraction in order to transform the code from \Cref{fig:atomicity:racy} into the one from \Cref{fig:atomicity:atomic}.
% 		The differences between the code snippets is set in bold font.
% 	}
% 	\label{fig:atomicity-intermediary-steps}
% \end{tcolorbox}
% \end{figure}

% \sw{Do we really want this example??}
% We revisit the above example and present the full reasoning.
% The first step is to identify $\guardof{\mathtt{head}, 0}{}$ to be a mover.
% Applying this mover results in the code from \Cref{fig:atomicity-intermediary-steps:protect}.
% Next, we want to move the assignment to $\mathtt{head}$ as well.
% However, it is not a right-mover since an interfering thread could change the valuation of the shared $\mathtt{Head}$ pointer.
% Instead, we let the assignment to $\mathtt{head}$ assign an non-deterministic value, see \Cref{fig:atomicity-intermediary-steps:nondet}.
% Now, the assignment does move as it is no longer affected by actions of interfering threads (since $\mathtt{head}$ is a local variable).
% We arrive at the code from \Cref{fig:atomicity-intermediary-steps:assign}.
% In this iteration, the non-deterministic assignment in the $\mathtt{else}$ has to assign to $\mathtt{head}$ the value of $\mathtt{Head}$ for the subsequent assumption to go through.
% Hence, we can replace the non-deterministic assignment with the original assignment using $\mathtt{Head}$.
% The result can be found in \Cref{fig:atomicity-intermediary-steps:oldassignagain}.
% As a last step to arrive at \Cref{fig:atomicity:atomic}, we can drop the now unnecessary assumption in the $\mathtt{else}$ branch.
% Moreover, the simulation argument from above allows us to deduce that removing the protection in the $\mathtt{if}$ allows for more behavior.
% Similarly, dropping the assumption in the same branch allows for more behavior.
% Lastly, a live-variables analysis reveals that $\mathtt{head}$ is not used and can thus be dropped as well.




==> content/_unused_prf_full.tex <==
%!TEX root = ../main.tex

\presection
\section{Getting Rid of Memory Reclamation}
\label{sec:prf}

\todoi{%
	Der Leser versteht noch nicht: Wieso hat SMR soviel Einfluss auf die Semantik.
	Das muss irgendwo hin.
	Verbunden damit: Warum ist Satz~\ref{thm:PRF-guarantee} wichtig. 
	Generell ist das noch eine etwas ungeführte Aneinanderreihung von Techniken.
}

Despite the compact formulation of SMR algorithms as SMR automata, analyzing programs in the presence of memory reclamation remains difficult.
The problem is that,
% unlike for programs relying on an automatic garbage collector,
unlike for programs running under garbage collection,
ownership guarantees~\cite{} and the resulting thread-local reasoning techniques~\cite{SeparationLogic} do not apply.
\Citet{DBLP:journals/pacmpl/MeyerW19} bridge this gap.
They have shown that it is sound and complete to conduct verification under garbage collection provided the program properly manages its memory.
So one can first establish this requirement and then perform the actual verification task under the simpler semantics.
Their statement is as follows; we will give the missing definitions in a moment.
%
\begin{theorem}[Consequence of Theorem 5.20 in \cite{DBLP:journals/pacmpl/MeyerW19}]
	\label{thm:PRF-guarantee}
	If the semantics $\anobs\freesem$ is pointer-race-free and generous, then $\anobs\allsem\computrel\nosem$.
\end{theorem}

We will argue below that the SMR automata for all major SMR algorithms guarantee generosity for all programs.
Hence, the only property to be checked in the presence of memory reclamation is the premise of pointer race freedom.
However, \citet{DBLP:journals/pacmpl/MeyerW19} report on this task being rather challenging, requiring an intricate state space exploration of a much more complicated semantics than garbage collection.
The contribution of the present paper is a type system to overcome exactly this challenge.



% =============================================================================================== %
% =============================================================================================== %
% =============================================================================================== %
\paragraph{Pointer Race Freedom}
Pointer races generalize the concept of memory errors by taking into account the SMR algorithm~\cite{DBLP:conf/vmcai/HazizaHMW16,DBLP:journals/pacmpl/MeyerW19}.
A memory error is an access through a dangling pointer, a pointer to an address that has been freed.
Such accesses are prone to system crashes, for example, due to segfaults.
Indeed, the \cppeleven standard considers programs with memory errors to have an undefined semantics (catch-fire semantics)~\cite{}.

To make precise which pointers in a computation are dangling, \citet{DBLP:conf/vmcai/HazizaHMW16} introduce the notion of \emph{validity}.
A pointer is then dangling if it is invalid.
Initially, all pointers are invalid.
A pointer is rendered valid if it receives its value from an allocation or from a valid pointer.
A pointer becomes invalid if its address is freed or it receives its value form an invalid pointer.
It is worth pointing out that $\freeof{\anadr}$ invalidates all pointers to address $\anadr$ but a subsequent reallocation of $\anadr$ validates only the receiving pointer.
We denote the set of valid pointers after a computation~$\tau$~by~$\validof{\tau}$.

We already argued that dereferences of invalid pointers may lead to system crashes.
Consequently, passing invalid pointers to the SMR algorithm may also be unsafe.
For an example, consider the call $\retireof{\apvar}$ requesting the SMR algorithm to free the address of $\apvar$.
If $\apvar$ is invalid, then its address has already been freed, resulting in a system crash due to a double-free.
However, we cannot forbid invalid pointers from being passed to SMR functions at all.
For instance, $\guard$ may be invoked with invalid pointers in \Cref{code:michaelscott_hp:protect-tail,code:michaelscott_hp:protect-head} of Michael\&Scott's queue from \Cref{sec:illustration}.
To support such calls, we deem a command $\enterof{\afuncof{\vecof{\apvar},\vecof{\advar}}}$ unsafe, if replacing the actual values of invalid pointer arguments with arbitrary values may exhibit (potentially undesired) SMR behavior that is not observed by the actual call.
%
\begin{definition}
	\label{def:unsafe-enter}
	Consider computation $\tau.\anact$. Action $\anact$ is an \emph{unsafe call} if its command is of the form $\enterof{\afuncof{\vecof{\apvar},\vecof{\advar}}}$ with $\apvar_i\notin\validof{\tau}$ for some $i$, ${\heapcomputof{\tau}{\vecof{\apvar}}=\vecof{\anadr}}$, $\heapcomputof{\tau}{\vecof{\advar}}=\vecof{\advalue}$, and:
	\begin{align*}
		\exists\,\anadrpp~
		\exists\,\vecof{\anadrp}.~~
		\big(
			\forall i.~ 
			(
			\anadr_i=\anadrpp\vee\apvar_i\in\validof{\tau}
			)
			\implies
			\anadr_i=\anadrp_i
		\big)
		\wedge
		\freeableof{\ahist.\afunc(\athread,\vecof{\anadrp},\vecof{\advalue})}{\anadrpp}
		\not\subseteq
		\freeableof{\ahist.\afunc(\athread,\vecof{\anadr},\vecof{\advalue})}{\anadrpp}
		\ .
	\end{align*}
\end{definition}

\begin{definition}
	\label{def:prf-brief}
	A computation $\tau.\anact$ is a \emph{pointer race} if $\anact$
	\begin{inparaenum}[(i)]
		\item dereferences an invalid pointer,
		\item is an assumption comparing an invalid pointer for equality,
		\item retires an invalid pointer, or
		\item is an unsafe call.
	\end{inparaenum}
\end{definition}

With this definition in place, the idea of our type system from \Cref{sec:type_system} is to syntactically under-approximate the set of valid pointers.
We use this under-approximation to establish pointer race freedom.


% =============================================================================================== %
% =============================================================================================== %
% =============================================================================================== %
\paragraph{Generosity}
% A semantics is generous if the program is not required \sw{die frees sind ja eigentlich nichts was das Programm macht} to give back addresses to the runtime environment in the following sense: without excuting free commands the SMR automaton may admit more behavior. 
% \sw{finde den Satz verwirrend.}
A semantics is generous if the program does not require the SMR algorithm to return retired addresses to the runtime environment.
That is, no computation is restricted by the SMR algorithm delaying frees rather than performing them eagerly.
%
\begin{definition}
	The semantics $\anobs\freesem$ is \emph{generous} if for all $\tau\in \anobs\freesem$ with history $\ahist.\freeof{\anadr}$ we have $\specof{\ahist.\freeof{\anadr}}\subseteq\specof{\ahist}$.
\end{definition}

We give a criterion on SMR automata that guarantees generosity for all programs.
It is satisfied by all SMR algorithms we considered.

\begin{lemma}
	Assume $\freeableof{\ahist.\freeof{\anadr}}{\anadr}\subseteq\freeableof{\ahist}{\anadr}$ for all histories $\ahist$ and some address $\anadr$.
	Then the semantics $\anobs\freesem$ is generous, for every program $\aprog$.
\end{lemma}

In the following, we use generosity to remove from a computation without re-allocations all $\free$ actions.
This allows us to bring the verification to the garbage collection semantics.
\sw{Man könnte überlegen die Generosity in die Elisions-Definition zu packen. Da haben wir sowas ähnliches, es sollte kaum auffallen. Hier ist es ein kurzer Einschub, der ggf. nicht 100\% klar wird.}


% =============================================================================================== %
% =============================================================================================== %
% =============================================================================================== %
\paragraph{Reduction}
\Cref{thm:PRF-guarantee} establishes a reduction of the behavior of full $\anobs\smash{\allsem}$ to the behavior of the simpler, garbage collected semantics $\nosem$.
More precisely, it states that we find for every computation $\tau\in\anobs\allsem$ another computation $\sigma\in\nosem$ such that $\tau\computrel\sigma$.
We say that $\sigma$ mimics $\tau$.
In this case, $\tau$ and $\sigma$ agree on the control locations of threads and the valid memory of $\tau$.
(Technically, $\sigma$ cannot free memory and thus cannot invalidate expressions like $\tau$ can.)
That is, any pointer-race-free action after $\tau$ has the same effect after $\sigma$.
Put differently, threads cannot distinguish whether they are executing in $\tau$ or $\sigma$.
So they cannot distinguish whether or not memory is reclaimed.

Our result from above follows from Theorem 5.20 in \cite{DBLP:journals/pacmpl/MeyerW19}.
Theorem 5.20 only assumes pointer race freedom and shows $\anobs\allsem\computrel\anobs\poplsem{\anadr}$.
Semantics $\anobs\poplsem{\anadr}$ allows for arbitrary frees but avoids re-allocations except for address $\anadr$.
Their proof strategy \cite{DBLP:journals/corr/MeyerW19} allows for a straight forward lift to $\anobs\allsem\computrel\anobs\freesem$ (cf. \Cref{thm:elision-computations-new} in the appendix).
Now, generosity removes frees altogether.
As a result, we can apply verification tools for GC to derive information about the program behavior with memory reclamation.

Technically, generosity justifies $\anobs\freesem\computrel\nosem$.
To see this, consider $\tau\in \anobs\freesem$.
We drop the actions which execute $\freeof{\anadr}$ and obtain the computation $\sigma$.
The threads will not react to the absence of frees.
By generosity, this will also not affect the SMR automaton.
Hence, $\sigma\in\anobs\nosem$ which equals $\nosem$ by Lemma~\ref{Lemma:GC}.
% (For a more formal discussion, refer to \Cref{thm:deletable-computations}.)

While the above extension follows easily, the main challenge remains: establishing pointer race freedom.
We address this challenge with a type system in the next section.


% % =============================================================================================== %
% % =============================================================================================== %
% % =============================================================================================== %
% \paragraph{Equivalence}
% \sw{---oben eine alternative Version---}
% The equivalence in \Cref{thm:PRF-guarantee} indicates that for every computation $\tau\in\anobs\allsem$ there is a computation $\sigma\in\nosem$ with $\tau\computrel\sigma$, and vice versa. 
% Two computations $\tau$ and $\sigma$ are similar if they agree on the control locations of threads, on the valid memory, and on the invariant formulas (up to logical equivalence). \sw{was hat es hier mit den invarianten auf sich? Brauchen wir hier nicht.}
% %The valid memory of $\tau$, denoted by $\vmem{\tau}$, is a restriction of $\heapcomput{\tau}$ to the valid pointer expressions, the data variables, and the data selectors of all addresses that are referenced by at least one valid pointer. 

% Our result follows from Theorem 5.20 in \cite{DBLP:journals/pacmpl/MeyerW19}.
% Theorem 5.20 only assumes pointer race freedom and shows $\anobs\allsem\computequiv\anobs\sem{\aprog}_{\set{\anadr}}^\emptyset$ \sw{nope. shows: $\anobs\allsem\computequiv\anobs\poplsem{\anadr}$}. 
% Semantics $\anobs\sem{\aprog}_{\set{\anadr}}^\emptyset$ avoids reallocations but still frees one address. 
% This address requires us to take into account the SMR automaton when verifying the program.  
% Generosity removes frees altogether.  
% As a result, we can apply verification tools for GC to derive information about the program behavior under memory reclamation.
% \sw{Das klingt nach einem starken Resultat, welches hier nebenbei abgehandelt wird. Die Challenge ist Pointer Races zu finden, ohne eine Semantik die frees macht zu exploren. In related news: tatsächlich haben wir eine bisschen stärkere validity Definition, weshalb wir auch rewriting machen müssen; das umgeht das POPL Paper durch 1 Reallokation.}

% Technically, generosity justifies $\anobs\freesem\computequiv\nosem$. 
% To see this, consider $\tau\in \anobs\freesem$. 
% We drop the actions $\freeof{\anadr}$ and obtain a computation $\sigma$. 
% The threads will not react to the absence of frees. 
% By generosity, this will also not affect the SMR automaton. 
% Hence, $\sigma\in\anobs\nosem$ which equals $\nosem$ by Lemma~\ref{Lemma:GC}.
% By definition, the frees do not have an influence on the invariants. 

%  \rfm{No PRF needed?}\sw{Yap, see: \Cref{thm:deletable-computations}.}

%  \todoi{Hier geht $\computequiv$ und $\computrel$ durcheinander.}



==> content/figures/benchmarks_old.tex <==
%!TEX root = ../../main.tex

% Table
\begin{table}%
\begin{tcolorbox}
	\caption{Experimental results for verifying singly-linked data structures using hazard pointers. The experiments were conducted on an Intel i5-8600K@3.6GHz with 16GB of RAM.}%
	\label{table:benchmarks}%
	\begin{minipage}{\columnwidth}
		\center%
		\newcommand{\cellSpacer}{\hspace{3mm}}
		\newcommand{\widthLeft}{.7cm}
		\newcommand{\widthRight}{.6cm}
		\newcommand{\cellDunno}[1]{\makebox[\widthLeft][r]{\(#1\)}\cellSpacer\makebox[\widthRight][l]{\rawsymbolTO}}
		\newcommand{\cellTO}{\makebox[\widthLeft][r]{---}\cellSpacer\makebox[\widthRight][l]{\rawsymbolTO}}
		\newcommand{\cellYes}[1]{\makebox[\widthLeft][r]{\(#1\)}\cellSpacer\makebox[\widthRight][l]{\rawsymbolYes}}
		\newcommand{\cellNo}[2][]{\makebox[\widthLeft][r]{\(#2\)}\cellSpacer\makebox[\widthRight][l]{\rawsymbolNo#1}}
		\newcommand{\seprule}{\midrule[.2pt]}
		\begin{tabularx}{\textwidth}{lXcccc}%
			\toprule
			SMR
				&Program
				& man. Types
				& gen. Types
				% \footnote{%
				% 	For HP, the synthesis took $28s$ and produced $315$ guarantees.
				% 	For EBR, it took $1s$ and produced $9$ guarantees.}
				& Annotations
				& Lineariz.
				\\
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\midrule
			\multirow{8}{*}{HP}
			&Treiber's stack
				& \cellYes{1.2s}
				& \cellYes{26s}
				& \cellYes{12s}
				& \cellYes{1s}
				\\
			&Opt. Treiber's stack
				& \cellYes{0.8s}
				& \cellYes{19s}
				& \cellYes{11s}
				& \cellYes{1s}
				\\
			&Michael\&Scott's queue
				& \cellYes{2.3s}
				& \cellYes{63s}
				& \cellYes{12s}
				& \cellYes{4s}
				\\
			&DGLM queue
				& \cellYes{42.3s}
				& \cellYes{23s}
				& \cellNo[\footnote{False-positive due to imprecision in the back-end verifier.\label{footnote:imprecision}}]{1s}
				& \cellYes{5s}
				\\
			&Vechev\&Yahav DCAS set
				& \cellYes{11s}
				& \cellYes{230s}
				& \cellYes{13s}
				& \cellYes{98s}
				\\
			&Vechev\&Yahav CAS set
				& \cellYes{11s}
				& \cellYes{205s}
				& \cellYes{3.5h} %$12518s$
				& \cellYes{42m} %$2470.24s$
				\\
			&ORVYY set
				& \cellYes{11s}
				& \cellYes{205s}
				& \cellYes{3.2h} %$11498s$
				& \cellYes{47m} %$2737.27s$
				\\
			&Michael's set
				& \cellYes{23s}
				& \cellYes{479s}
				& \cellNo[\textsuperscript{\ref{footnote:imprecision}}]{90s}
				& \cellTO
				\\
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\midrule
			\multirow{8}{*}{EBR}
			&Treiber's stack
				& \cellYes{0.12s}
				& \cellYes{0.16s}
				& \cellYes{10s}
				& \cellYes{1s}
				\\
			&Opt. Treiber's stack
				& \cellYes{0.12s}
				& \cellYes{0.16s}
				& \cellYes{12s}
				& \cellYes{1s}
				\\
			&Michael\&Scott's queue
				& \cellYes{0.18s}
				& \cellYes{0.18s}
				& \cellYes{16s}
				& \cellYes{5s}
				\\
			&DGLM queue
				& \cellYes{0.17s}
				& \cellYes{0.19s}
				& \cellNo[\textsuperscript{\ref{footnote:imprecision}}]{1s}
				& \cellYes{6s}
				\\
			&Vechev\&Yahav DCAS set
				& \cellYes{0.23s}
				& \cellYes{0.25s}
				& \cellYes{38s}
				& \cellYes{200s}
				\\
			&Vechev\&Yahav CAS set
				& \cellYes{0.21s}
				& \cellYes{0.23s}
				& \cellYes{7h}%25446.28s
				& \cellYes{42m}% 2513.11s
				\\
			&ORVYY set
				& \cellYes{0.21s}
				& \cellYes{0.23s}
				& \cellYes{7h}%23886.88s
				& \cellYes{47m}%2797.70s
				\\
			&Michael's set
				& \cellYes{0.48s}
				& \cellYes{0.51s}
				& \cellNo[\textsuperscript{\ref{footnote:imprecision}}]{22s}
				& \cellTO
				\\
			\bottomrule
		\end{tabularx}
	\end{minipage}
\end{tcolorbox}
\end{table}


==> content/types_example.tex <==
%!TEX root = ../main.tex

\subsection{Example (old)}
\label{sec:type_system:example}

We revisit the type checking example from \Cref{sec:illustration}.
The type derivation is given in \Cref{fig:typing-example}.
The goal is to derive in our type system that \code{head} is successfully protected.
For simplicity, we give in the type environments in \Cref{fig:typing-example} only the pointers \code{Head} and \code{head}.
The remaining pointers are also present but do not affect our example.

\begin{myfloatfigure}[r]{5.4cm}
\begin{lstlisting}[style=typing]
`{ Head:$\emptyset$, head:$\emptyset$ }`
  Node* head = Head;
`{ Head:$\emptyset$, head:$\emptyset$ }`
  enter protect(head, 0);
`{ Head:$\emptyset$, head:$\gilluinv$ }`
  exit protect;
`{ Head:$\emptyset$, head:$\gilluisu$ }`
  beginAtomic;
`{ Head:$\emptyset$, head:$\gilluisu$ }`
  @inv active(Head)
`{ Head:$\gactive$, head:$\gilluisu$ }`
  assume(head == Head);
`{ Head:$\gactive\wedge\gilluisu$, head:$\gactive\wedge\gilluisu$ }`
`{ Head:$\gactive\wedge\gilluisu$, head:$\gactive\wedge\gilluisu\wedge\gsafeaccess$ }`
  endAtomic;
`{ Head:$\emptyset$, head:$\gilluisu\wedge\gsafeaccess$ }`
\end{lstlisting}%
	\caption{%
		Type check of \Cref{code:michaelscott:read-head,code:michaelscott:protect-head,code:michaelscott:check-head} for a successful protection of \code{head}.
		\rev{add line numbers wrt. Fig. 2}
	}
	\label{fig:typing-example}
\end{myfloatfigure}%
%
In the beginning, the type of \code{Head} and \code{head} is $\emptyset$.
There are no guarantees.
The first command assigns the value of \code{Head} to \code{head}.
We apply Rule~\ref{rule:assign1}.
Both pointers continue to have type $\emptyset$.
Next, \code{protect} is invoked with \code{head} as a parameter.
Using Rule~\ref{rule:enter} we obtain type $\gilluinv$ for \code{head}, stating that we have definitely invoked \code{protect} for \code{head}.
The type of \code{Head} is not affected.
After \code{protect} returns, \code{head} obtains type $\gilluisu$ from an application of Rule~\ref{rule:exit}.
It encodes the fact that a protection has been issued.
Accessing \code{head}, however, is not safe at this point since we do not know whether \code{head}
has been retired in the meantime.
Next, we enter an atomic section, it has no effect on the types as of Rule~\ref{rule:begin}.
The subsequent active annotation adds $\gactive$ to the type of \code{Head}, Rule~\ref{rule:active}.
Guarantee $\gactive$ is maintained because we are inside an atomic block.
The following assumption conjoins the types of \code{Head} and \code{head}, Rule~\ref{rule:assume1}.
The result is $\gactive\wedge\gilluisu$.
An application of Rule~\ref{rule:infer} allows us to infer $\gsafeaccess$ for \code{head}.
To this end, we perform an inclusion check among the corresponding locations, $\locsof{\gactive}\cap\locsof{\gilluisu}\subseteq \locsof{\gsafeaccess}$, as required by the transformer relation $\leadsto$.
We could also infer $\gsafeaccess$ for \code{Head}, but the guarantee will be removed when leaving the atomic section.
Finally, Rule~\ref{rule:end} updates the types to account for interference after leaving the atomic section.
The type of \code{Head} is set to $\emptyset$ and and $\gactive$ is removed from \code{head}.
The point to note here is that \code{head} maintains $\gsafeaccess$.
That is, subsequent accesses are guaranteed to be safe.

